Order Matters: 3D Shape Generation from Sequential VR Sketches

VR sketching lets users explore and iterate on ideas directly in 3D, offering a faster and more intuitive alternative to conventional CAD tools. However, existing sketch-to-shape models ignore the temporal ordering of strokes, discarding crucial cues about structure and design intent. We introduce VRSketch2Shape, the first framework and multi-category dataset for generating 3D shapes from sequential VR sketches. Our contributions are threefold: (i) an automated pipeline that generates sequential VR sketches from arbitrary shapes, (ii) a dataset of over 20k synthetic and 900 hand-drawn sketch-shape pairs across four categories, and (iii) an order-aware sketch encoder coupled with a diffusion-based 3D generator. Our approach yields higher geometric fidelity than prior work, generalizes effectively from synthetic to real sketches with minimal supervision, and performs well even on partial sketches. All data and models will be released open-source at https://chenyizi086.github.io/VRSketch2Shape_website.

==> figures/chair.tex <==



\tikzset{
  point/.style={
    circle,                     % node shape
    ball color=blue!70!black,   % gradient “ball” shading
    shading angle=210,           % light direction → change for effect
    inner sep= \pointsize pt,              % dot size
    postaction={draw=white!80!black,line width=.5pt,opacity=.5,
    minimum height=0mm} % tiny highlight
  },
 edge/.style={
   smooth,
   line width=\linewidthcustom pt,
   tension=0.5
  },
}

  \node[anchor=south west, inner sep=0, opacity=0] (img) at (0,0)
    {\includegraphics[width=\wsketch cm]{images/pipeline/chair_sketch.jpg}};

    \useasboundingbox (img.south west) rectangle (img.north east);


  \begin{scope}[shift={(img.south west)},
                x={(img.south east)},
                y={(img.north west)}]

    \node[point,  ball color=ball1] (p1) at (0.15,0.1,0.1) {};
    \node[point,  ball color=ball2] (p2) at (0.18,0.1,1) {};
    \node[point,  ball color=ball3] (p3) at (0.13,0.1,2) {};
    \node[point,  ball color=ball4] (p4) at (0.5,0.1,2.2) {};

    \node[point,  ball color=ball5] (p5) at (0.6,0.1,-0.1) {};
    \node[point,  ball color=ball6] (p6) at (0.6,0.1,0.6) {};

    \node[point,  ball color=ball7] (p7) at (0.9,0.1,-0.0) {};
    \node[point,  ball color=ball8] (p8) at (0.9,0.1,0.9) {};
    \node[point,  ball color=ball9] (p9) at (0.5,0.1,1.2) {};

\draw[line width=\linewidthcustom pt, edge1]    plot[edge] coordinates { (p5) (p6) (p2) };
\draw[line width=\linewidthcustom pt, edge2]   plot[edge] coordinates { (p1) (p2) (p3) (p4) };
\draw[line width=\linewidthcustom pt, edge3]  plot[edge] coordinates { (p7) (p8) (p9) (p4) };
\draw[line width=\linewidthcustom pt, edge4] plot[edge] coordinates { (p2) (p9) };
\draw[line width=\linewidthcustom pt, edge5]   plot[edge] coordinates { (p6) (p8) };


    \node[point,  ball color=ball1] (p1) at (0.15,0.1,0.1) {};
    \node[point,  ball color=ball2] (p2) at (0.18,0.1,1) {};
    \node[point,  ball color=ball3] (p3) at (0.13,0.1,2) {};
    \node[point,  ball color=ball4] (p4) at (0.5,0.1,2.2) {};

    \node[point,  ball color=ball5] (p5) at (0.6,0.1,-0.1) {};
    \node[point,  ball color=ball6] (p6) at (0.6,0.1,0.6) {};

    \node[point,  ball color=ball7] (p7) at (0.9,0.1,-0.0) {};
    \node[point,  ball color=ball8] (p8) at (0.9,0.1,0.9) {};
    \node[point,  ball color=ball9] (p9) at (0.5,0.1,1.2) {};
    
  \end{scope}

==> figures/chair_sketch_1.tex <==
%auto-ignore
\def\pointsize{3}%
\def\linewidthcustom{3}
\definecolor{edge1}{RGB}{210,210,210}%   % bright blue
\definecolor{edge2}{RGB}{210,210,210}%     % vivid red
\definecolor{edge3}{RGB}{210,210,210}% %  % vibrant green
\definecolor{edge4}{RGB}{210,210,210}%  % warm orange
\definecolor{edge5}{RGB}{210,210,210}%    % bright cyan
\definecolor{ball1}{RGB}{200,200,200}%
\definecolor{ball2}{RGB}{200,200,200}%
\definecolor{ball3}{RGB}{200,200,200}%
\definecolor{ball4}{RGB}{200,200,200}%
\definecolor{ball5}{RGB}{255,0,0}%
\definecolor{ball6}{RGB}{200,200,200}%
\definecolor{ball7}{RGB}{200,200,200}%
\definecolor{ball8}{RGB}{200,200,200}%
\definecolor{ball9}{RGB}{200,200,200}%
\begin{tikzpicture}[tdplot_main_coords]
\input{figures/chair}
\draw[line width=\linewidthcustom pt, edgehighlight1]   plot[edge] coordinates { (p5) (p6) (p2) };
\node[point,  ball color=ball5]  at (p5.center) {};
\node[point,  ball color=ball6] at (p6.center) {};
\node[point,  ball color=ball2] at (p2.center) {};
\end{tikzpicture}

==> figures/chair_sketch_2.tex <==
\def\pointsize{3}%
\def\linewidthcustom{3}
\definecolor{edge1}{RGB}{210,210,210}%   % bright blue
\definecolor{edge2}{RGB}{210,210,210}%     % vivid red
\definecolor{edge3}{RGB}{210,210,210}% %  % vibrant green
\definecolor{edge4}{RGB}{210,210,210}%  % warm orange
\definecolor{edge5}{RGB}{210,210,210}%    % bright cyan
\definecolor{ball1}{RGB}{200,200,200}%
\definecolor{ball2}{RGB}{200,200,200}%
\definecolor{ball3}{RGB}{200,200,200}%
\definecolor{ball4}{RGB}{200,200,200}%
\definecolor{ball5}{RGB}{200,200,200}%
\definecolor{ball6}{RGB}{255,0,0}%
\definecolor{ball7}{RGB}{200,200,200}%
\definecolor{ball8}{RGB}{200,200,200}%
\definecolor{ball9}{RGB}{200,200,200}%
\begin{tikzpicture}[tdplot_main_coords]
\input{figures/chair}
\draw[line width=\linewidthcustom pt, edgehighlight1]   plot[edge] coordinates { (p5) (p6) (p2) };
\node[point,  ball color=ball5]  at (p5.center) {};
\node[point,  ball color=ball6] at (p6.center) {};
\node[point,  ball color=ball2] at (p2.center) {};
\end{tikzpicture}

==> figures/chair_sketch_3.tex <==
\def\pointsize{3}%
\def\linewidthcustom{3}
\definecolor{edge1}{RGB}{210,210,210}%   % bright blue
\definecolor{edge2}{RGB}{210,210,210}%     % vivid red
\definecolor{edge3}{RGB}{210,210,210}% %  % vibrant green
\definecolor{edge4}{RGB}{210,210,210}%  % warm orange
\definecolor{edge5}{RGB}{210,210,210}%    % bright cyan
\definecolor{ball1}{RGB}{200,200,200}%
\definecolor{ball2}{RGB}{255,0,0}%
\definecolor{ball3}{RGB}{200,200,200}%
\definecolor{ball4}{RGB}{200,200,200}%
\definecolor{ball5}{RGB}{200,200,200}%
\definecolor{ball6}{RGB}{200,200,200}%
\definecolor{ball7}{RGB}{200,200,200}%
\definecolor{ball8}{RGB}{200,200,200}%
\definecolor{ball9}{RGB}{200,200,200}%
\begin{tikzpicture}[tdplot_main_coords]
\input{figures/chair}
\draw[line width=\linewidthcustom pt, edgehighlight1]   plot[edge] coordinates { (p5) (p6) (p2) };
\node[point,  ball color=ball6]  at (p6.center) {};
\node[point,  ball color=ball2] at (p2.center) {};
\node[point,  ball color=ball5]  at (p5.center) {};
\end{tikzpicture}

==> figures/chair_sketch_4.tex <==
\def\pointsize{3}%
\def\linewidthcustom{3}
\definecolor{edge1}{RGB}{210,210,210}%   % bright blue
\definecolor{edge2}{RGB}{210,210,210}%     % vivid red
\definecolor{edge3}{RGB}{210,210,210}% %  % vibrant green
\definecolor{edge4}{RGB}{210,210,210}%  % warm orange
\definecolor{edge5}{RGB}{210,210,210}%    % bright cyan
\definecolor{ball1}{RGB}{255,0,0}%
\definecolor{ball2}{RGB}{200,200,200}%
\definecolor{ball3}{RGB}{200,200,200}%
\definecolor{ball4}{RGB}{200,200,200}%
\definecolor{ball5}{RGB}{200,200,200}%
\definecolor{ball6}{RGB}{200,200,200}%
\definecolor{ball7}{RGB}{200,200,200}%
\definecolor{ball8}{RGB}{200,200,200}%
\definecolor{ball9}{RGB}{200,200,200}%
\begin{tikzpicture}[tdplot_main_coords]
\input{figures/chair}
\draw[line width=\linewidthcustom pt, edgehighlight2]   plot[edge] coordinates { (p1) (p2) (p3) (p4)};
\node[point,  ball color=ball1]  at (p1.center) {};
\node[point,  ball color=ball2] at (p2.center) {};
\node[point,  ball color=ball3]  at (p3.center) {};
\node[point,  ball color=ball4] at (p4.center) {};
\end{tikzpicture}

==> figures/chair_sketch_5.tex <==
\def\pointsize{3}%
\def\linewidthcustom{3}
\definecolor{edge1}{RGB}{210,210,210}%   % bright blue
\definecolor{edge2}{RGB}{210,210,210}%     % vivid red
\definecolor{edge3}{RGB}{210,210,210}% %  % vibrant green
\definecolor{edge4}{RGB}{210,210,210}%  % warm orange
\definecolor{edge5}{RGB}{210,210,210}%    % bright cyan
\definecolor{ball1}{RGB}{200,200,200}%
\definecolor{ball2}{RGB}{255,0,0}%
\definecolor{ball3}{RGB}{200,200,200}%
\definecolor{ball4}{RGB}{200,200,200}%
\definecolor{ball5}{RGB}{200,200,200}%
\definecolor{ball6}{RGB}{200,200,200}%
\definecolor{ball7}{RGB}{200,200,200}%
\definecolor{ball8}{RGB}{200,200,200}%
\definecolor{ball9}{RGB}{200,200,200}%
\begin{tikzpicture}[tdplot_main_coords]
\input{figures/chair}
\draw[line width=\linewidthcustom pt, edgehighlight2]   plot[edge] coordinates { (p1) (p2) (p3) (p4)};
\node[point,  ball color=ball1]  at (p1.center) {};
\node[point,  ball color=ball2] at (p2.center) {};
\node[point,  ball color=ball3]  at (p3.center) {};
\node[point,  ball color=ball4] at (p4.center) {};
\end{tikzpicture}

==> figures/chair_sketch_main.tex <==
\def\pointsize{1}%
\def\linewidthcustom{1}
\definecolor{edge1}{RGB}{160,25,140}% 
\definecolor{edge2}{RGB}{160,120,130}% 
\definecolor{edge3}{RGB}{150,160,170}% 
\definecolor{edge4}{RGB}{110,175,120}% 
\definecolor{edge5}{RGB}{185,175,50}% 
\definecolor{ball1}{RGB}{0,50,200}%
\definecolor{ball2}{RGB}{0,50,200}%
\definecolor{ball3}{RGB}{0,50,200}%
\definecolor{ball4}{RGB}{0,50,200}%
\definecolor{ball5}{RGB}{0,50,200}%
\definecolor{ball6}{RGB}{0,50,200}%
\definecolor{ball7}{RGB}{0,50,200}%
\definecolor{ball8}{RGB}{0,50,200}%
\definecolor{ball9}{RGB}{0,50,200}%
\begin{tikzpicture}[tdplot_main_coords]
\input{figures/chair}
\end{tikzpicture}


%    rgb255(0cm)=(185,175,50), 
%    rgb255(1cm)=(110,175,120),
%%    rgb255(2cm)=(150,160,170),
%    rgb255(3cm)=(160,120,130) ,
%    rgb255(4cm)=(160,25,140),

==> tables/models.tex <==
\begin{tabular}{l ccccc}\toprule
     & code & pretraining & order of  \\
     & available  & modality & strokes  \\\midrule
  Chen & no & images & no \\\greyrule 
  Luo   & yes &  point cloud & no\\\greyrule 
  us    &  yes & SoS & yes & \\\bottomrule
\end{tabular}
